Sign Language Recognition via Skeleton-Aware Multi-Model Ensemble

Sign language is commonly used by deaf or mute people to communicate but requires extensive effort to master. It is usually performed with the fast yet delicate movement of hand gestures, body posture, and even facial expressions. Current Sign Language Recognition (SLR) methods usually extract features via deep neural networks and suffer overfitting due to limited and noisy data. Recently, skeleton-based action recognition has attracted increasing attention due to its subject-invariant and background-invariant nature, whereas skeleton-based SLR is still under exploration due to the lack of hand annotations. Some researchers have tried to use off-line hand pose trackers to obtain hand keypoints and aid in recognizing sign language via recurrent neural networks. Nevertheless, none of them outperforms RGB-based approaches yet. To this end, we propose a novel Skeleton Aware Multi-modal Framework with a Global Ensemble Model (GEM) for isolated SLR (SAM-SLR-v2) to learn and fuse multi-modal feature representations towards a higher recognition rate. Specifically, we propose a Sign Language Graph Convolution Network (SL-GCN) to model the embedded dynamics of skeleton keypoints and a Separable Spatial-Temporal Convolution Network (SSTCN) to exploit skeleton features. The skeleton-based predictions are fused with other RGB and depth based modalities by the proposed late-fusion GEM to provide global information and make a faithful SLR prediction. Experiments on three isolated SLR datasets demonstrate that our proposed SAM-SLR-v2 framework is exceedingly effective and achieves state-of-the-art performance with significant margins. Our code will be available at https://github.com/jackyjsy/SAM-SLR-v2

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/songyao_bio.pdf}}]{Songyao Jiang}
received his B.Eng. degree in electrical engineering in Hong Kong Polytechnic University at 2013, and M.S. degree in electrical and computer engineering from University of Michigan, Ann Arbor MI at 2015. He is currently pursuing his Ph.D. degree in computer engineering at Northeastern University, Boston MA. His current research interests include human detection, pose estimation, face recognition, skeleton-based action recognition, sign language recognition, and generative adversarial networks. He has served as PC member and reviewer for many journals and conferences including ICCV, IJCAI, FG, ICDM, MIPR, TIP, JEI, JVCI etc. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/binsun_bio.pdf}}]{Bin Sun} received the B.Eng. degree in photoelectric information engineering from Beijing Institute of Technology (BIT), China, in 2015. He is pursuing the Ph.D. degree with the Department of Electrical and Computer Engineering, Northeastern University, Boston, MA, USA. His research interests include Face Synthesis and light weight network design. He has served as PC member for AAAI, and published paper in AAAI 2018, BMVC 2018, FG 2020.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/lichenwang_bio.pdf}}]{Lichen Wang}(S'16) received the B.Eng. degree in Automation from Harbin Institute of Technology, Harbin, China in 2013. The M.Eng. degree with the Department of Electronic Science and Engineering from Xi'an Jiaotong University, Xi'an, China in 2016. The Ph.D. degree with the Department of Electrical and Computer Engineering, Northeastern University, Boston, USA. His research interests include computer vision, machine learning, multi-label learning, multi-view learning, domain adaptation, and graph representation learning. Dr. Wang has served as the reviewer for journals and conferences including TPAMI, TIP, TNNLS, CVPR, ICCV, ECCV, IJCAI, AAAI, ICLR, NeurIPS, and ICML.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yuebai_bio.pdf}}]{Yue Bai} received the B.Sc. degree in Mathematics from Donghua University, Shanghai, China in 2017. And the M.Eng. degree in Data Analytics Engineering from Northeastern University, Boston, MA, the USA in 2019. He is currently pursuing the Ph.D. degree with the Department of Electrical and Computer Engineering,  Northeastern University, Boston, MA, USA. His research interests include computer vision, machine learning, and deep learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/kunpeng_bio.pdf}}]{Kunpeng Li} (S'18) received the B.Eng. degree in Information Engineering from South China University of Technology, China, the Ph.D. degree with the Department of Electrical and Computer Engineering, Northeastern University, Boston, USA. His research interests include weakly-supervised learning, scene understanding, vision and language, video analytics. He has spent time at Google AI Research, Bytedance AI Lab, Adobe Research, Siemens Research as a research intern. He has received Outstanding Graduate Research Award and Dean's Fellowship from College of Engineering, Northeastern University. He has served as Program Committee Members or reviewers for many AI conferences and journals, e.g. CVPR, ICCV, ECCV, NeurIPS, ICLR, ICML, TPAMI, IJCV, TIP, etc.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/Yun.pdf}}]{Yun Fu} (S’07-M’08-SM’11-F’19) received the
B.Eng. degree in information engineering and the
M.Eng. degree in pattern recognition and intelligence
systems from Xian Jiaotong University, China,
respectively, and the M.S. degree in statistics and
the Ph.D. degree in electrical and computer engineering
from the University of Illinois at Urbana-
Champaign, respectively. He is an interdisciplinary
faculty member affiliated with Khoury College of
Computer Sciences at Northeastern University since
2012. His research interests are Machine Learning,
Computational Intelligence, Big Data Mining, Computer Vision, Pattern
Recognition, and Cyber-Physical Systems. He has extensive publications in
leading journals, books/book chapters and international conferences/workshops.
He serves as associate editor, chairs, PC member and reviewer of many
top journals and international conferences/workshops. He received seven
Prestigious Young Investigator Awards from NAE, ONR, ARO, IEEE, INNS,
UIUC, Grainger Foundation; eleven Best Paper Awards from IEEE, ACM,
IAPR, SPIE, SIAM; many major Industrial Research Awards from Google,
Amazon, Samsung, MERL, Konica Minolta, JP Morgan, Zebra, Adobe, and
Mathworks, etc. He is currently an Associate Editor of the IEEE Transactions
on Image Processing (TIP) and ACM Transactions on Knowledge Discovery
from Data (TKDD). He is fellow of IEEE, IAPR, OSA and SPIE, lifetime
Distinguished member of ACM, Lifetime Senior Member of AAAI and Institute
of Mathematical Statistics, member of ACM Future of Computing Academy,
Global Young Academy, AAAS, INNS and Beckman Graduate Fellow during
2007-2008.
\end{IEEEbiography}
